Angular analysis of the $B^{0}\rightarrow K^{*0}\mu^{+}\mu^{-}$ decay using $3\,\mbox{fb}^{-1}$ of integrated luminosity

An angular analysis of the $B^{0}\rightarrow K^{*0}(\rightarrow K^{+}\pi^{-})\mu^{+}\mu^{-}$ decay is presented. The dataset corresponds to an integrated luminosity of $3.0\,{\mbox{fb}^{-1}}$ of $pp$ collision data collected at the LHCb experiment. The complete angular information from the decay is used to determine $C\!P$-averaged observables and $C\!P$ asymmetries, taking account of possible contamination from decays with the $K^{+}\pi^{-}$ system in an S-wave configuration. The angular observables and their correlations are reported in bins of $q^2$, the invariant mass squared of the dimuon system. The observables are determined both from an unbinned maximum likelihood fit and by using the principal moments of the angular distribution. In addition, by fitting for $q^2$-dependent decay amplitudes in the region $1.1<q^{2}<6.0\mathrm{\,Ge\kern -0.1em V}^{2}/c^{4}$, the zero-crossing points of several angular observables are computed. A global fit is performed to the complete set of $C\!P$-averaged observables obtained from the maximum likelihood fit. This fit indicates differences with predictions based on the Standard Model at the level of 3.4 standard deviations. These differences could be explained by contributions from physics beyond the Standard Model, or by an unexpectedly large hadronic effect that is not accounted for in the Standard Model predictions.

==> LHCb_HD_comma_separated_author_2015-10-13.tex <==
LHCb collaboration:
R. Aaij, 
C. Abell\'{a}n Beteta, 
B. Adeva, 
M. Adinolfi, 
A. Affolder, 
Z. Ajaltouni, 
S. Akar, 
J. Albrecht, 
F. Alessio, 
M. Alexander, 
S. Ali, 
G. Alkhazov, 
P. Alvarez Cartelle, 
A.A. Alves Jr, 
S. Amato, 
S. Amerio, 
Y. Amhis, 
L. An, 
L. Anderlini, 
G. Andreassi, 
M. Andreotti, 
J.E. Andrews, 
R.B. Appleby, 
O. Aquines Gutierrez, 
F. Archilli, 
P. d'Argent, 
A. Artamonov, 
M. Artuso, 
E. Aslanides, 
G. Auriemma, 
M. Baalouch, 
S. Bachmann, 
J.J. Back, 
A. Badalov, 
C. Baesso, 
W. Baldini, 
R.J. Barlow, 
C. Barschel, 
S. Barsuk, 
W. Barter, 
V. Batozskaya, 
V. Battista, 
A. Bay, 
L. Beaucourt, 
J. Beddow, 
F. Bedeschi, 
I. Bediaga, 
L.J. Bel, 
V. Bellee, 
N. Belloli, 
I. Belyaev, 
E. Ben-Haim, 
G. Bencivenni, 
S. Benson, 
J. Benton, 
A. Berezhnoy, 
R. Bernet, 
A. Bertolin, 
M.-O. Bettler, 
M. van Beuzekom, 
S. Bifani, 
P. Billoir, 
T. Bird, 
A. Birnkraut, 
A. Bizzeti, 
T. Blake, 
F. Blanc, 
J. Blouw, 
S. Blusk, 
V. Bocci, 
A. Bondar, 
N. Bondar, 
W. Bonivento, 
S. Borghi, 
M. Borisyak, 
M. Borsato, 
T.J.V. Bowcock, 
E. Bowen, 
C. Bozzi, 
S. Braun, 
M. Britsch, 
T. Britton, 
J. Brodzicka, 
N.H. Brook, 
E. Buchanan, 
C. Burr, 
A. Bursche, 
J. Buytaert, 
S. Cadeddu, 
R. Calabrese, 
M. Calvi, 
M. Calvo Gomez, 
P. Campana, 
D. Campora Perez, 
L. Capriotti, 
A. Carbone, 
G. Carboni, 
R. Cardinale, 
A. Cardini, 
P. Carniti, 
L. Carson, 
K. Carvalho Akiba, 
G. Casse, 
L. Cassina, 
L. Castillo Garcia, 
M. Cattaneo, 
Ch. Cauet, 
G. Cavallero, 
R. Cenci, 
M. Charles, 
Ph. Charpentier, 
M. Chefdeville, 
S. Chen, 
S.-F. Cheung, 
N. Chiapolini, 
M. Chrzaszcz, 
X. Cid Vidal, 
G. Ciezarek, 
P.E.L. Clarke, 
M. Clemencic, 
H.V. Cliff, 
J. Closier, 
V. Coco, 
J. Cogan, 
E. Cogneras, 
V. Cogoni, 
L. Cojocariu, 
G. Collazuol, 
P. Collins, 
A. Comerma-Montells, 
A. Contu, 
A. Cook, 
M. Coombes, 
S. Coquereau, 
G. Corti, 
M. Corvo, 
B. Couturier, 
G.A. Cowan, 
D.C. Craik, 
A. Crocombe, 
M. Cruz Torres, 
S. Cunliffe, 
R. Currie, 
C. D'Ambrosio, 
E. Dall'Occo, 
J. Dalseno, 
P.N.Y. David, 
A. Davis, 
O. De Aguiar Francisco, 
K. De Bruyn, 
S. De Capua, 
M. De Cian, 
J.M. De Miranda, 
L. De Paula, 
P. De Simone, 
C.-T. Dean, 
D. Decamp, 
M. Deckenhoff, 
L. Del Buono, 
N. D\'{e}l\'{e}age, 
M. Demmer, 
D. Derkach, 
O. Deschamps, 
F. Dettori, 
B. Dey, 
A. Di Canto, 
F. Di Ruscio, 
H. Dijkstra, 
S. Donleavy, 
F. Dordei, 
M. Dorigo, 
A. Dosil Su\'{a}rez, 
A. Dovbnya, 
K. Dreimanis, 
L. Dufour, 
G. Dujany, 
K. Dungs, 
P. Durante, 
R. Dzhelyadin, 
A. Dziurda, 
A. Dzyuba, 
S. Easo, 
U. Egede, 
V. Egorychev, 
S. Eidelman, 
S. Eisenhardt, 
U. Eitschberger, 
R. Ekelhof, 
L. Eklund, 
I. El Rifai, 
Ch. Elsasser, 
S. Ely, 
S. Esen, 
H.M. Evans, 
T. Evans, 
M. Fabianska, 
A. Falabella, 
C. F\"{a}rber, 
N. Farley, 
S. Farry, 
R. Fay, 
D. Ferguson, 
V. Fernandez Albor, 
F. Ferrari, 
F. Ferreira Rodrigues, 
M. Ferro-Luzzi, 
S. Filippov, 
M. Fiore, 
M. Fiorini, 
M. Firlej, 
C. Fitzpatrick, 
T. Fiutowski, 
F. Fleuret, 
K. Fohl, 
P. Fol, 
M. Fontana, 
F. Fontanelli, 
D. C. Forshaw, 
R. Forty, 
M. Frank, 
C. Frei, 
M. Frosini, 
J. Fu, 
E. Furfaro, 
A. Gallas Torreira, 
D. Galli, 
S. Gallorini, 
S. Gambetta, 
M. Gandelman, 
P. Gandini, 
Y. Gao, 
J. Garc\'{i}a Pardi\~{n}as, 
J. Garra Tico, 
L. Garrido, 
D. Gascon, 
C. Gaspar, 
R. Gauld, 
L. Gavardi, 
G. Gazzoni, 
D. Gerick, 
E. Gersabeck, 
M. Gersabeck, 
T. Gershon, 
Ph. Ghez, 
S. Gian\`{i}, 
V. Gibson, 
O.G. Girard, 
L. Giubega, 
V.V. Gligorov, 
C. G\"{o}bel, 
D. Golubkov, 
A. Golutvin, 
A. Gomes, 
C. Gotti, 
M. Grabalosa G\'{a}ndara, 
R. Graciani Diaz, 
L.A. Granado Cardoso, 
E. Graug\'{e}s, 
E. Graverini, 
G. Graziani, 
A. Grecu, 
E. Greening, 
P. Griffith, 
L. Grillo, 
O. Gr\"{u}nberg, 
B. Gui, 
E. Gushchin, 
Yu. Guz, 
T. Gys, 
T. Hadavizadeh, 
C. Hadjivasiliou, 
G. Haefeli, 
C. Haen, 
S.C. Haines, 
S. Hall, 
B. Hamilton, 
X. Han, 
S. Hansmann-Menzemer, 
N. Harnew, 
S.T. Harnew, 
J. Harrison, 
J. He, 
T. Head, 
V. Heijne, 
A. Heister, 
K. Hennessy, 
P. Henrard, 
L. Henry, 
J.A. Hernando Morata, 
E. van Herwijnen, 
M. He\ss, 
A. Hicheur, 
D. Hill, 
M. Hoballah, 
C. Hombach, 
W. Hulsbergen, 
T. Humair, 
M. Hushchyn, 
N. Hussain, 
D. Hutchcroft, 
D. Hynds, 
M. Idzik, 
P. Ilten, 
R. Jacobsson, 
A. Jaeger, 
J. Jalocha, 
E. Jans, 
A. Jawahery, 
M. John, 
D. Johnson, 
C.R. Jones, 
C. Joram, 
B. Jost, 
N. Jurik, 
S. Kandybei, 
W. Kanso, 
M. Karacson, 
T.M. Karbach, 
S. Karodia, 
M. Kecke, 
M. Kelsey, 
I.R. Kenyon, 
M. Kenzie, 
T. Ketel, 
E. Khairullin, 
B. Khanji, 
C. Khurewathanakul, 
T. Kirn, 
S. Klaver, 
K. Klimaszewski, 
O. Kochebina, 
M. Kolpin, 
I. Komarov, 
R.F. Koopman, 
P. Koppenburg, 
M. Kozeiha, 
L. Kravchuk, 
K. Kreplin, 
M. Kreps, 
P. Krokovny, 
F. Kruse, 
W. Krzemien, 
W. Kucewicz, 
M. Kucharczyk, 
V. Kudryavtsev, 
A. K. Kuonen, 
K. Kurek, 
T. Kvaratskheliya, 
D. Lacarrere, 
G. Lafferty, 
A. Lai, 
D. Lambert, 
G. Lanfranchi, 
C. Langenbruch, 
B. Langhans, 
T. Latham, 
C. Lazzeroni, 
R. Le Gac, 
J. van Leerdam, 
J.-P. Lees, 
R. Lef\`{e}vre, 
A. Leflat, 
J. Lefran\c{c}ois, 
E. Lemos Cid, 
O. Leroy, 
T. Lesiak, 
B. Leverington, 
Y. Li, 
T. Likhomanenko, 
M. Liles, 
R. Lindner, 
C. Linn, 
F. Lionetto, 
B. Liu, 
X. Liu, 
D. Loh, 
I. Longstaff, 
J.H. Lopes, 
D. Lucchesi, 
M. Lucio Martinez, 
H. Luo, 
A. Lupato, 
E. Luppi, 
O. Lupton, 
A. Lusiani, 
F. Machefert, 
F. Maciuc, 
O. Maev, 
K. Maguire, 
S. Malde, 
A. Malinin, 
G. Manca, 
G. Mancinelli, 
P. Manning, 
A. Mapelli, 
J. Maratas, 
J.F. Marchand, 
U. Marconi, 
C. Marin Benito, 
P. Marino, 
J. Marks, 
G. Martellotti, 
M. Martin, 
M. Martinelli, 
D. Martinez Santos, 
F. Martinez Vidal, 
D. Martins Tostes, 
L.M. Massacrier, 
A. Massafferri, 
R. Matev, 
A. Mathad, 
Z. Mathe, 
C. Matteuzzi, 
A. Mauri, 
B. Maurin, 
A. Mazurov, 
M. McCann, 
J. McCarthy, 
A. McNab, 
R. McNulty, 
B. Meadows, 
F. Meier, 
M. Meissner, 
D. Melnychuk, 
M. Merk, 
E Michielin, 
D.A. Milanes, 
M.-N. Minard, 
D.S. Mitzel, 
J. Molina Rodriguez, 
I.A. Monroy, 
S. Monteil, 
M. Morandin, 
P. Morawski, 
A. Mord\`{a}, 
M.J. Morello, 
J. Moron, 
A.B. Morris, 
R. Mountain, 
F. Muheim, 
D. M\"{u}ller, 
J. M\"{u}ller, 
K. M\"{u}ller, 
V. M\"{u}ller, 
M. Mussini, 
B. Muster, 
P. Naik, 
T. Nakada, 
R. Nandakumar, 
A. Nandi, 
I. Nasteva, 
M. Needham, 
N. Neri, 
S. Neubert, 
N. Neufeld, 
M. Neuner, 
A.D. Nguyen, 
T.D. Nguyen, 
C. Nguyen-Mau, 
V. Niess, 
R. Niet, 
N. Nikitin, 
T. Nikodem, 
A. Novoselov, 
D.P. O'Hanlon, 
A. Oblakowska-Mucha, 
V. Obraztsov, 
S. Ogilvy, 
O. Okhrimenko, 
R. Oldeman, 
C.J.G. Onderwater, 
B. Osorio Rodrigues, 
J.M. Otalora Goicochea, 
A. Otto, 
P. Owen, 
A. Oyanguren, 
A. Palano, 
F. Palombo, 
M. Palutan, 
J. Panman, 
A. Papanestis, 
M. Pappagallo, 
L.L. Pappalardo, 
C. Pappenheimer, 
W. Parker, 
C. Parkes, 
G. Passaleva, 
G.D. Patel, 
M. Patel, 
C. Patrignani, 
A. Pearce, 
A. Pellegrino, 
G. Penso, 
M. Pepe Altarelli, 
S. Perazzini, 
P. Perret, 
L. Pescatore, 
K. Petridis, 
A. Petrolini, 
M. Petruzzo, 
E. Picatoste Olloqui, 
B. Pietrzyk, 
M. Pikies, 
D. Pinci, 
A. Pistone, 
A. Piucci, 
S. Playfer, 
M. Plo Casasus, 
T. Poikela, 
F. Polci, 
A. Poluektov, 
I. Polyakov, 
E. Polycarpo, 
A. Popov, 
D. Popov, 
B. Popovici, 
C. Potterat, 
E. Price, 
J.D. Price, 
J. Prisciandaro, 
A. Pritchard, 
C. Prouve, 
V. Pugatch, 
A. Puig Navarro, 
G. Punzi, 
W. Qian, 
R. Quagliani, 
B. Rachwal, 
J.H. Rademacker, 
M. Rama, 
M. Ramos Pernas, 
M.S. Rangel, 
I. Raniuk, 
N. Rauschmayr, 
G. Raven, 
F. Redi, 
S. Reichert, 
A.C. dos Reis, 
V. Renaudin, 
S. Ricciardi, 
S. Richards, 
M. Rihl, 
K. Rinnert, 
V. Rives Molina, 
P. Robbe, 
A.B. Rodrigues, 
E. Rodrigues, 
J.A. Rodriguez Lopez, 
P. Rodriguez Perez, 
S. Roiser, 
V. Romanovsky, 
A. Romero Vidal, 
J. W. Ronayne, 
M. Rotondo, 
T. Ruf, 
P. Ruiz Valls, 
J.J. Saborido Silva, 
N. Sagidova, 
B. Saitta, 
V. Salustino Guimaraes, 
C. Sanchez Mayordomo, 
B. Sanmartin Sedes, 
R. Santacesaria, 
C. Santamarina Rios, 
M. Santimaria, 
E. Santovetti, 
A. Sarti, 
C. Satriano, 
A. Satta, 
D.M. Saunders, 
D. Savrina, 
S. Schael, 
M. Schiller, 
H. Schindler, 
M. Schlupp, 
M. Schmelling, 
T. Schmelzer, 
B. Schmidt, 
O. Schneider, 
A. Schopper, 
M. Schubiger, 
M.-H. Schune, 
R. Schwemmer, 
B. Sciascia, 
A. Sciubba, 
A. Semennikov, 
A. Sergi, 
N. Serra, 
J. Serrano, 
L. Sestini, 
P. Seyfert, 
M. Shapkin, 
I. Shapoval, 
Y. Shcheglov, 
T. Shears, 
L. Shekhtman, 
V. Shevchenko, 
A. Shires, 
B.G. Siddi, 
R. Silva Coutinho, 
L. Silva de Oliveira, 
G. Simi, 
M. Sirendi, 
N. Skidmore, 
T. Skwarnicki, 
E. Smith, 
E. Smith, 
I.T. Smith, 
J. Smith, 
M. Smith, 
H. Snoek, 
M.D. Sokoloff, 
F.J.P. Soler, 
F. Soomro, 
D. Souza, 
B. Souza De Paula, 
B. Spaan, 
P. Spradlin, 
S. Sridharan, 
F. Stagni, 
M. Stahl, 
S. Stahl, 
S. Stefkova, 
O. Steinkamp, 
O. Stenyakin, 
S. Stevenson, 
S. Stoica, 
S. Stone, 
B. Storaci, 
S. Stracka, 
M. Straticiuc, 
U. Straumann, 
L. Sun, 
W. Sutcliffe, 
K. Swientek, 
S. Swientek, 
V. Syropoulos, 
M. Szczekowski, 
T. Szumlak, 
S. T'Jampens, 
A. Tayduganov, 
T. Tekampe, 
G. Tellarini, 
F. Teubert, 
C. Thomas, 
E. Thomas, 
J. van Tilburg, 
V. Tisserand, 
M. Tobin, 
J. Todd, 
S. Tolk, 
L. Tomassetti, 
D. Tonelli, 
S. Topp-Joergensen, 
N. Torr, 
E. Tournefier, 
S. Tourneur, 
K. Trabelsi, 
M. Traill, 
M.T. Tran, 
M. Tresch, 
A. Trisovic, 
A. Tsaregorodtsev, 
P. Tsopelas, 
N. Tuning, 
A. Ukleja, 
A. Ustyuzhanin, 
U. Uwer, 
C. Vacca, 
V. Vagnoni, 
G. Valenti, 
A. Vallier, 
R. Vazquez Gomez, 
P. Vazquez Regueiro, 
C. V\'{a}zquez Sierra, 
S. Vecchi, 
M. van Veghel, 
J.J. Velthuis, 
M. Veltri, 
G. Veneziano, 
M. Vesterinen, 
B. Viaud, 
D. Vieira, 
M. Vieites Diaz, 
X. Vilasis-Cardona, 
V. Volkov, 
A. Vollhardt, 
D. Voong, 
A. Vorobyev, 
V. Vorobyev, 
C. Vo\ss, 
J.A. de Vries, 
R. Waldi, 
C. Wallace, 
R. Wallace, 
J. Walsh, 
J. Wang, 
D.R. Ward, 
N.K. Watson, 
D. Websdale, 
A. Weiden, 
M. Whitehead, 
J. Wicht, 
G. Wilkinson, 
M. Wilkinson, 
M. Williams, 
M.P. Williams, 
M. Williams, 
T. Williams, 
F.F. Wilson, 
J. Wimberley, 
J. Wishahi, 
W. Wislicki, 
M. Witek, 
G. Wormser, 
S.A. Wotton, 
K. Wraight, 
S. Wright, 
K. Wyllie, 
Y. Xie, 
Z. Xu, 
Z. Yang, 
J. Yu, 
X. Yuan, 
O. Yushchenko, 
M. Zangoli, 
M. Zavertyaev, 
L. Zhang, 
Y. Zhang, 
A. Zhelezov, 
A. Zhokhov, 
L. Zhong, 
V. Zhukov, 
S. Zucchelli

